Replicability Measures for Longitudinal Information Retrieval Evaluation

Information Retrieval (IR) systems are exposed to constant changes in most components. Documents are created, updated, or deleted, the information needs are changing, and even relevance might not be static. While it is generally expected that the IR systems retain a consistent utility for the users, test collection evaluations rely on a fixed experimental setup. Based on the LongEval shared task and test collection, this work explores how the effectiveness measured in evolving experiments can be assessed. Specifically, the persistency of effectiveness is investigated as a replicability task. It is observed how the effectiveness progressively deteriorates over time compared to the initial measurement. Employing adapted replicability measures provides further insight into the persistence of effectiveness. The ranking of systems varies across retrieval measures and time. In conclusion, it was found that the most effective systems are not necessarily the ones with the most persistent performance.

==> tables/results.tex <==
% \setlength\extrarowheight{2.2pt}
\begin{tabular}{cc|cccc|cccc|cccc}
    \toprule
 & & \multicolumn{4}{c|}{P@10} & \multicolumn{4}{c|}{bpref} & \multicolumn{4}{c}{nDCG} \\
 & & ARP & $\mathcal{R}_e\Delta$ & $\Delta$RI & ER & ARP & $\mathcal{R}_e\Delta$ & $\Delta$RI & ER & ARP & $\mathcal{R}_e\Delta$ & $\Delta$RI & ER \\\midrule

\multirow[c]{3}{*}{\rotatebox{90}{\scriptsize BM25}} & WT & 0.095 & 0 & - & - & 0.314 & 0 & - & - & 0.269 & 0 & - & - \\
 & ST & 0.089 & 0.064 & - & - & 0.314 & -0.002 & - & - & 0.272 & -0.010 & - & - \\
 & LT & 0.110 & -0.165 & - & - & 0.324 & -0.033 & - & - & 0.306 & -0.137 & - & - \\\midrule

\multirow[c]{3}{*}{\rotatebox{90}{\scriptsize ColBERT}} & WT & 0.097 & 0 & 0 & 1 & 0.324 & 0 & 0 & 1 & 0.276 & 0 & 0 & 1 \\
 & ST & 0.094 & 0.028 & -0.040 & 2.540 & 0.317 & 0.022 & 0.024 & 0.286 & 0.275 & 0.004 & 0.015 & 0.441 \\
 & LT & 0.120 & -0.238 & -0.064 & 4.355 & 0.338 & -0.041 & -0.008 & 1.278 & 0.297 & -0.078 & 0.053 & -1.198 \\ \midrule

\multirow[c]{3}{*}{\rotatebox{90}{\scriptsize MonoT5}} & WT & 0.106 & 0 & 0 & 1 & 0.337 & 0 & 0 & 1 & 0.295 & 0 & 0 & 1 \\
 & ST & 0.109 & -0.028 & -0.110 & 1.815 & 0.344 & -0.019 & -0.019 & 1.261 & 0.302 & -0.023 & -0.013 & 1.146 \\
 & LT & 0.123 & -0.165 & 0.000 & 1.161 & 0.337 & 0.000 & 0.034 & 0.553 & 0.311 & -0.051 & 0.083 & 0.187 \\\midrule

\multirow[c]{3}{*}{\rotatebox{90}{\scriptsize RRF}} & WT & 0.101 & 0 & 0 & 1 & 0.346 & 0 & 0 & 1 & 0.285 & 0 & 0 & 1 \\
 & ST & 0.090 & 0.110 & 0.052 & 0.242 & 0.328 & 0.054 & 0.032 & 0.574 & 0.282 & 0.009 & 0.003 & 0.925 \\
 & LT & 0.121 & -0.192 & -0.025 & 1.573 & 0.347 & -0.004 & 0.002 & 1.007 & 0.314 & -0.105 & 0.013 & 0.786 \\\midrule

\multirow[c]{3}{*}{\rotatebox{90}{\scriptsize d2q}} & WT & 0.106 & 0 & 0 & 1 & 0.335 & 0 & 0 & 1 & 0.285 & 0 & 0 & 1 \\
 & ST & 0.104 & 0.018 & -0.056 & 1.379 & 0.331 & 0.013 & 0.015 & 0.779 & 0.287 & -0.005 & 0.006 & 0.916 \\
 & LT & 0.123 & -0.165 & 0.000 & 1.161 & 0.368 & -0.098 & -0.067 & 2.034 & 0.327 & -0.147 & -0.010 & 1.317 \\ \midrule

\multirow[c]{3}{*}{\rotatebox{90}{\scriptsize E5}} & WT & 0.096 & 0 & 0 & 1 & 0.368 & 0 & 0 & 1 & 0.290 & 0 & 0 & 1 \\
 & ST & 0.092 & 0.038 & -0.029 & 4.355 & 0.354 & 0.037 & 0.045 & 0.738 & 0.300 & -0.034 & -0.025 & 1.333 \\
 & LT & 0.123 & -0.291 & -0.109 & 17.419 & 0.371 & -0.008 & 0.028 & 0.863 & 0.313 & -0.080 & 0.054 & 0.362 \\
 \bottomrule
\end{tabular}

